A framework for robotic arm pose estimation and movement prediction based on deep and extreme learning models

Human-robot collaboration has gained a notable prominence in Industry 4.0, as the use of collaborative robots increases efficiency and productivity in the automation process. However, it is necessary to consider the use of mechanisms that increase security in these environments, as the literature reports that risk situations may exist in the context of human-robot collaboration. One of the strategies that can be adopted is the visual recognition of the collaboration environment using machine learning techniques, which can automatically identify what is happening in the scene and what may happen in the future. In this work, we are proposing a new framework that is capable of detecting robotic arm keypoints commonly used in Industry 4.0. In addition to detecting, the proposed framework is able to predict the future movement of these robotic arms, thus providing relevant information that can be considered in the recognition of the human-robot collaboration scenario. The proposed framework is based on deep and extreme learning machine techniques. Results show that the proposed framework is capable of detecting and predicting with low error, contributing to the mitigation of risks in human-robot collaboration.

==> sections/intro-objcontr-OLD.tex <==
\subsection{Objective of this work and contributions}

Considering the previously identified research gaps, the need for safe in HRC and the promising high accuracy of DL models for detection tasks, the present work develops and evaluates a new framework for the accurate detection of robot poses and the prediction of future movement. The proposed framework consists of the following two parts:

\begin{enumerate}
    \item Robotic arm pose estimation: relies on re-training a CNN model named SCNet-50-V1-d \cite{liu2020improving} for the pose detection task of the robot through regression. The SCNet-50-V1-d model uses self-calibrated convolutions (SCConvs) and enjoyed a great deal of success in a wide range of application including image classification, object detection and instance segmentation. In this work, we also demonstrate the efficacy of using SCConvs for regression tasks. In addition, we improve pose estimation through the use of the extreme learning machine (ELM) neural network \cite{huang2006extreme}, which when combined with CNN models tends to provide a better learning outcome \cite{rodrigues2021convolutional}.
    \item Robotic arm movement prediction: contemplates the training a long-short term memory (LSTM) \cite{hochreiter1997long} and gated recurrent unit (GRU) models \cite{cho-etal-2014-learning} to predict the future movement of a robotic arm.
\end{enumerate}

Although this work contributes to risk mitigation is a HRC, it does not claim solving the  collision risk problem in its entirety. Our goal is to address the open gaps previously presented and propose a new framework that mainly provides future movement prediction and detect the pose of the robotic arm. This last mentioned step can be essential for risk assessment in the HRC context. The use of this framework allows for example a human agent to know where a robot will move to, providing it ample time for making decisions and reacting in order to remain safe and avoid any damage to a moving robot and humans nearby.

The framework is instantiated with several DL models that support pose detection and prediction of future robot movement. These are evaluated and compared in a well-controlled scenario, as defined by Silva et al. \cite{silva2020assessing}. Despite being a well-controlled setting, the adopted testbed includes real equipment such as the UR-5 robotic arm, networking and RBS devices installed in a rack. The scenario also inserts a person  responsible for performing collaborative activities with the robotic arm. These activities are recorded through a strategically positioned camera. We also annotate the data to carry out the regression of the robot's keypoints and obtain the current robot pose. We compared all the evaluated models using the two performance metrics: mean squared error (MSE) and mean absolute error (MAE) metrics. The obtained result demonstrate the suitability of using the proposed framework as an efficient solution for the detection and prediction of the future movement of a robotic arm while suffering a very low error.


%enfatizar o que tem de diferente nosso paper em relação ao estado da arte
%enfatizar TODAS as contribuições do nosso paper (como no JCAE)
Considering the current state-of-art, we can cite the following main contributions of our work:
\begin{itemize}
    %a proposta em si
    \item This work develops a new framework designed to predict robotic arm pose detection and its future movement in the context of HRC using DL, ELM and one 2D camera in a well controlled scenario.
    
    %cenário
    \item Our framework is applied and evaluated in the proposed controlled setup that highly mimics a real scenario, generating real data during the experiments for analysis. Unlike most existing related works, this one did not used synthetic images, e.g. robot located in random scenarios. It is also important to highlight that in our experiments the camera calibration process was not necessary. The additional steps part of the calibration processr, such as checkerboard position, camera positioning, acquisition of intrinsic and extrinsic parameters are error sensitive. Our goal is to use a generic environment where we could use devices present in-loco.
    
    %CELM (SCNet+ELM)
    \item To the best of our knowledge, this work is first to use ELM to solve a regression problem using features generated by a neural network that uses self-calibrated convolutions (SCNet). It is first to obtain robot pose detection using a convolutional extreme learning machine (CELM) approach. We demonstrate through extensive experiments that the DL model SCNet50 used in conjunction with the ELM method provide better detection results in our scenario.
    
    %movimentação do robô no contexto HRI
    \item Another important contribution of this work is the proposition of deep learning models to predict the future movement of the robotic arm. Models of this type had not been previously proposed in the literature to tackle this problem. There are works that apply DL only to human movement prediction models in the HRI context. Using DL, it becomes possible to analyze the future movement of the robot. Furthermore, DL models will also be considered, as part of future work, in the analysis of collision risk between humans and robots.
    
    % fácil de implementar
    \item Finally, the last contribution of this work is that the proposed framework is easy to deploy. The testbed  relies on infrastructure that is commonly found in workspaces including cameras, robotics arms, and networking devices.
    
\end{itemize}


==> sections/intro-rl-OLD.tex <==
\subsection{Related works}
\label{sec:relatedWorks}


%% -->
%apresentar deep learning/machine learning como possível arma para solucionar este problema
Across the literature,there are several technologies that can actually contribute towards detecting and mitigating risks in HRC \cite{robla2017working}, \cite{lasota2017survey}, \cite{silva2020assessing}, \cite{zhang2020recurrent}, \cite{anvaripour2019collision}, \cite{maceira2020recurrent}. Among these, we highlight the special role of machine learning (ML), which provides intelligent systems to solve the most diverse engineering problems, including HRC. In particular, we draw the attention to an emerging subfield of ML in the literature, deep learning (DL) \cite{lecun2015deep}. DL has proven to beat the state of the art in solving most common problems involving ML, such as the image classification challenge in the ImageNet database \cite{deng2009imagenet}, \cite{tan2019efficientnet}. Furthermore, DL has gained notable prominence in regression, clustering, among other tasks, through its use of convolutional neural networks (CNN) \cite{liu2017survey} and recurrent neural networks (RNN) \cite{lipton2015critical}.

As a result, there are several approaches in the literature that use DL models for risk mitigation in HRC \cite{silva2020assessing}, \cite{sharkawy2020human}, \cite{park2020learning}. Nonetheless, many of the already listed works are limited to carrying out the immediate detection of collision events. They do not predict eminent risk situations before they happen. To reduce damage to workers and agents involved in close collaboration scenarios with robots, one should ideally train new models that predict risk situations and analyze relevant data to predict possible risks in a timely manner and prior to taking place\cite{zhang2020recurrent}, \cite{anvaripour2019collision}, \cite{maceira2020recurrent}.

The authors are of the view that there are limited contributions that take into consideration the detection of human intention to estimate the likelihood of future risks. Such works suffer from a limited scope as they focus on detecting human movement \cite{zhang2020recurrent}, \cite{anvaripour2019collision}, \cite{maceira2020recurrent} and do not combine this with robot detection and the analysis of its movement. Note however that there are literary works that tackle robotic arms detection in an isolated context. Unlike these, this study develops and evaluates detection mechanisms for robots to assess their proximity, speed, collision risks, future movement, etc., in a HRC scenario. These assessments should provide a more robust solution for risk mitigation in HRC. % (Section \ref{sec:relatedWorks}), however, with a limitation: there are no approaches for detecting future movement (prediction) of robotic arms.

Pose estimation (or detection) is widely used in several computer vision applications such as medical assistance, games, and human intention detection. All previously cited applications refer to human pose estimation. Human pose estimation consists of detecting the human body keypoints through regression models. In a similar view, robot pose estimation consists of detecting the robot keypoints through regression models, these keypoints are the joints that compose the robot skeleton. With the advance of deep learning studies, there has been a notable advance in robot pose detection with several CNN applications with different types of robots. Robot pose detection aims to obtain the keypoints which represent the robot joints, thus constituting its pose. Bellow, we present recent papers on robot pose detection using CNNs.

Miseikis et al. \cite{miseikis2018robot} present an approach for detecting robot poses in RGB images. Their method consists of a cascade of two different convolutional networks. The first network performs the segmentation of the robot, with an architecture reminiscent of AlexNet \cite{krizhevsky2012imagenet}. In contrast, the second network is responsible for mapping the robot's key points from the mask extracted with the first network. The UR-5 robotic arm pose detection reached an accuracy of 98.1\% and outperformed that of UR-3 and UR-10 with 93.1\% and 92.8\%, respectively. 
In a similar research, Mivseikis et al. \cite{mivseikis2018transfer} propose the use of transfer learning to detect various tasks (as \cite{miseikis2018robot}), including the detection of keypoints of another type of robot, the Kuka LBR iiwa. The approach achieved an accuacy of 97.3\% for detecting the new robot's masks. This demonstrates that transfer learning also contributes to detecting keypoints of robots, even though there are fewer examples used for training the neural network.

Zhou et al. \cite{zhou20193d} also propose an architecture for detecting the pose of robots from RGB images. The architecture is divided into two parts, Base-Net and Pose-Net. In Pose-Net, the positions of the keypoints in the image are initially estimated to guide training. Base-Net obtains the 3D position of the robot base by calculating the depth and using the robot base position in the image evaluated by proposed system. 

Lee et al. \cite{lee2020camera} present an approach to estimate the pose of the robot using a single RGB image. As with similar previous works, a convolutional network is used to detect the robot's keypoints in artificial images due to the lack of the availability of real data reported by the authors. However, unlike previous works, the projection of keypoints is in 2D. Perspective-n-point (PnP) is then used to retrieve the camera extrinsic, allowing the approach to dismiss the need from an offline calibration step from a single frame.

Heindl et al. \cite{heindl2019learning} use a recurrent convolutional network based on ConvGRU-type convolutions \cite{ballas2015delving}. Despite the promising approach and reaching a mean average precision or mAP (threshold 50\%) of 88.7\%, all images used in their entirety were artificially generated to train the proposed architecture. Although the paper presents inferences in authentic images, there are no experiments or other evidence that the proposed approach can work in real scenarios. The idea of using artificial images was also adopted in previous work \cite{heindl20193d} by the same authors in \cite{heindl2019learning}, however, the neural networks were modeled with vanilla convolutions this time.

With regard to robot pose detection, there is a need to consider the importance of robots' keypoints in the context of safety for human-robot collaboration. Note also that none of the reviewed works considers the analysis of robots' keypoints information into a recurrent neural network in order to classify or predict robots' movements. In a typical HRC scenario, it is necessary to understand and classify/predict the robot's intention. This approach should help to avoid or decrease the impacts of collision/accident events.

